QuTiP 5: The Quantum Toolbox in Python

QuTiP, the Quantum Toolbox in Python, has been at the forefront of open-source quantum software for the past 13 years. It is used as a research, teaching, and industrial tool, and has been downloaded millions of times by users around the world. Here we introduce the latest developments in QuTiP v5, which are set to have a large impact on the future of QuTiP and enable it to be a modern, continuously developed and popular tool for another decade and more. We summarize the code design and fundamental data layer changes as well as efficiency improvements, new solvers, applications to quantum circuits with QuTiP-QIP, and new quantum control tools with QuTiP-QOC. Additional flexibility in the data layer underlying all ``quantum objects'' in QuTiP allows us to harness the power of state-of-the-art data formats and packages like JAX, CuPy, and more. We explain these new features with a series of both well-known and new examples. The code for these examples is available in a static form on GitHub and as continuously updated and documented notebooks in the qutip-tutorials package.

==> enr_waveguide.tex <==
import numpy as np
import scipy.sparse as sp
import qutip as qt
from qutip.core.energy_restricted import EnrSpace

from tqdm import tqdm
import matplotlib.pyplot as plt
from mpl_setup import * 

import time as time
from numpy.random import RandomState
prng = RandomState(int(time.time()))


# ---------- Utility Functions ----------

def _enr_project_state(dims, excitations, state):
    """
    Generate a projector onto a Fock state representation in a excitation-number restricted
    state space.  
    """
    nstates, state2idx, idx2state = qt.enr_state_dictionaries(dims, excitations)
    a_op = sp.lil_matrix((nstates, nstates), dtype=np.complex128)

    try:
        n = state2idx[tuple(state)]
    except KeyError: 
        raise ValueError("The state tuple %s is not in the restricted "
                         "state space" % str(tuple(state)))
    a_op[n, n] = 1

    enr_dims = [EnrSpace(dims, excitations)] * 2
    return qt.Qobj(a_op, dims=enr_dims)


def _enr_project_sub_system(dims, excitations, mode, s0):
    """
    Projector onto a particular state in position "mode" with excitation s0
    E.g., mode=0, s0=1, excitations=2, returns |1,0><1,0| + |1,1><1,1|
    """
    nstates, state2idx, idx2state = qt.enr_state_dictionaries(dims, excitations)
    a_op = sp.lil_matrix((nstates, nstates), dtype=np.complex128)

    for n1, state1 in enumerate(list(idx2state.values())):
        for idx, s in enumerate(state1):
            # if s > 0, the annihilation operator of mode idx has a non-zero
            # entry with one less excitation in mode idx in the final state
            if idx == mode and s0==s:
                a_op[n1, n1] = 1

    enr_dims = [EnrSpace(dims, excitations)] * 2
    return qt.Qobj(a_op, dims=enr_dims)


def _enr_projector_subdim(dims, excitations, subrange, n_exc):
    """
    Generate the projector onto excitation subspace
    """
    nstates, state2idx, idx2state = qt.enr_state_dictionaries(dims, excitations)
    a_op = sp.lil_matrix((nstates, nstates), dtype=np.complex128)

    for n1, state1 in enumerate(list(idx2state.values())):
        if sum([state1[i] for i in subrange]) == n_exc:
            a_op[n1, n1] = 1

    enr_dims = [EnrSpace(dims, excitations)] * 2
    return qt.Qobj(a_op, dims=enr_dims)


# ---------- Solve problem ----------

def Waveguide_Solve(d, psi0, deltat, T, phi, N, wq=0, g=1, Ntraj=500):
    """
    A basic implementation of the space-discretized waveguide model from 
    Regidor et al, PHYSICAL REVIEW RESEARCH 3, 023030 (2021).
    Note this only implements a single qubit coupled to a waveguide
    truncated by a mirror at one end, and only in the single-excitation limit.

    Will evolve the state ("psi0") until time ("T") in steps ("deltat"),
    and average over ("Ntraj") iterations

    Parameters
    ----------

    d : list of [:obj:`.Qobj`] of length ("N+1"). d[0:-1] must be the
        annhilation operators defining the ("N") discrete waveguide modes
        and d[-1] must be the annilation operator for the system (qubit)

    psi0 : :obj:`.Qobj`
        initial state vector (ket). 

    deltat : float, simultaneously defines the time step used in the discrete
        propagation below and the length of the waveguide via L = deltat * N

    T : float, total integration time.

    phi : float, phase acquired at the mirror truncating the waveguide.

    N : int, number of modes.

    wq : float, qubit energy

    g : float, coupling strength

    Ntraj: int, number of trajectories used for averaging.

    Returns
    -------

    output_states: list of [:obj:`.Qobj`] representing the qubit+waveguide 
        states at all times in [0, T] in time-steps of deltat
    """

    # list of annihilation operators for cavity modes
    a = d[0:-1]

    # atomic annihilation operator
    sm = d[-1]

    #example of states:
    #a[0].dag()|0> = [1,0,0,0,0]
    #a[-1].dag()|0> = [0,0,0,1,0]
    #sm.dag()|0> = [0,0,0,0,1]

    H0 = wq * sm.dag() * sm

    #Atom-Waveguide couplings
    #left moving box
    Hint_ac = (
        (np.sqrt(g) / np.sqrt(2 * deltat)) *
        (a[0].dag() * sm + sm.dag() * a[0])
    )

    #right moving box.
    Hint_ac += (
        (np.sqrt(g) / np.sqrt(2 * deltat)) * 
        (np.exp(-1.0j * phi) * a[-1].dag() * sm +  
         np.exp(1.0j * phi) * sm.dag() * a[-1])
    )

    H = H0 + Hint_ac
   
    #Utility functions:
    #projector onto single excitation in the last right moving box
    coll_a = _enr_project_sub_system(dims, excitations, N-1, 1)  

    #projector onto the empty state in the right-moving box
    coll_0 = _enr_project_sub_system(dims, excitations, N-1, 0) 

    #propagator for interaction evolution
    U = (-1.0j * deltat * H).expm()

    #projector onto 1 photon subspace
    proj_1ss = _enr_projector_subdim(dims, excitations, np.arange(0,N), 1)

    #construct propagator for moving state between boxes
    U_shift1 = 0
    #Translates all excitations one space to the left every time step.
    #If more than one total excitations, this is insufficient.
    for n in range(N-1):
        U_shift1 += a[n+1].dag() * a[n]
    U_shift = U_shift1 * proj_1ss
    #this adds on projectors onto the 0 photon subspace, to make sure they are not projected out by U_shift:
    U_shift += (
        _enr_project_state(dims,excitations, [0 if m == (N) else 0 for m in range(N+1)]) +
        _enr_project_state(dims,excitations, [1 if m == (N) else 0 for m in range(N+1)])
    )

    # Do the simulation:

    Nsteps = int(np.round(T / deltat))
    output_states = [0 for _ in range(Nsteps+1)]
    output_states[0] = psi0 * psi0.dag()

    for traj in tqdm(range(Ntraj)):

        psi1 = psi0
        nt = 0
        for _ in range(Nsteps):
            nt += 1
            psi1 = U * psi1

            Pout = qt.expect(coll_a, psi1)
            numpa = prng.rand()

            if numpa <= Pout:
                psi1 = coll_a * psi1
                psi1 = a[-1] * psi1
            else:
                psi1 = (coll_0) * psi1

            psi1 = U_shift * psi1
            psi1 = psi1.unit()

            output_states[nt] += psi1 * psi1.dag() / Ntraj

    return output_states


N = 21      # number of waveguide modes
M = 2       # normal, assumed, mode fock-state truncation
wq = 0.     # qubit frequency
g = 1       # coupling constant

#Physical dimensions of the qubit+waveguide modes
dims = [M] * N + [2]
#Restricted number of excitations in the qubit+waveguide modes
excitations = 1           # total number of excitations
initial_excitiations = 1  # initial number of excitations

#Construct ENR operators and states
d = qt.enr_destroy(dims, excitations)
psi0 = qt.enr_fock(dims, excitations, [initial_excitiations if m == N else 0 for m in range(N+1)])

deltat = 1 / (N-1)  #set up so that it arrives back to interact with system at t=(N-1)deltat
T=5  #total integration time

phi = np.pi #phase change at mirror
output_states_phipi = Waveguide_Solve(d, psi0, deltat, T, phi, N,
                                      wq, g,Ntraj = 4000)

phi = 0 #phase change at mirror
output_states_phi0 = Waveguide_Solve(d, psi0, deltat, T, phi, N,
                                     wq, g,Ntraj = 4000)


# ---------- Generate plots ----------

Nsteps = int(np.round(T / deltat))
times = np.linspace(0, T, Nsteps + 1)

plt.figure()
#plt.plot(times, [1/np.e for t in times])
plt.plot(times, qt.expect(d[-1].dag()*d[-1], output_states_phipi), label= r"With mirror, $\phi=\pi$")
plt.plot(times, qt.expect(d[-1].dag()*d[-1], output_states_phi0),'--', label= r"With mirror, $\phi=0$")
plt.plot(times, [(np.cos(np.sqrt(g*deltat/2))**(2*n) * np.exp(-(g/2) * n * deltat))  for n in range(Nsteps+1)], ':',label="Without mirror")

plt.legend(loc=0)
plt.xlabel(r"$t$ $(1/\gamma$)", fontsize=18)
plt.ylabel("TLS Population", fontsize=18)

plt.savefig("enr_waveguide_mirror.pdf")
plt.show()

from mpl_toolkits.mplot3d import Axes3D
from matplotlib import cm
e_ops = [x.dag() * x for x in d[0:-1]]
mode_occup_listphi0 = []
for tk,t in enumerate(times):
    mode_occup = []
    for kk in range(N):
        mode_occup.append(qt.expect(e_ops[kk],output_states_phi0[len(times)-tk-1]))
    mode_occup_listphi0.append(mode_occup)

mode_occup_listphipi = []
for tk,t in enumerate(times):
    mode_occup = []
    for kk in range(N):
        mode_occup.append(qt.expect(e_ops[kk],output_states_phipi[len(times)-tk-1]))
    mode_occup_listphipi.append(mode_occup)

X, Y = np.meshgrid(range(len(mode_occup_listphi0[0])),times[::-1])


fig = plt.figure(figsize=plt.figaspect(1.5))
fig.subplots_adjust(wspace=0, hspace=-0.15)

ax = fig.add_subplot(211, projection='3d')
ax.zaxis.set_rotate_label(False) 
ax.zaxis.set_label_position('top')
ax.plot_surface(X, -Y,np.array(mode_occup_listphi0), rstride=1, cstride=1, cmap=cm.viridis, alpha=0.9)
ax.set_yticks([-2,-4],["2","4"])
ax.tick_params(axis="y", pad=6)
ax.tick_params(axis="z", pad=8)
ax.tick_params(axis="x", pad=4)
ax.set_ylabel("t $(1/\gamma)$")
ax.set_xlabel("n")
#ax.set_zlabel("$B_n^{\dagger}B_n$")

ax.set_box_aspect((4,4,2))
ax.yaxis.labelpad=10
ax.zaxis.labelpad=5
ax.xaxis.labelpad=10
#plt.savefig("waveguide_phi0.pdf")


ax = fig.add_subplot(212, projection='3d')
ax.zaxis.set_rotate_label(False) 
ax.plot_surface(X, -Y,np.array(mode_occup_listphipi), rstride=1, cstride=1, cmap=cm.viridis, alpha=0.9)
ax.set_yticks([-2,-4],["2","4"])
ax.tick_params(axis="y", pad=6)
ax.tick_params(axis="z", pad=8)
ax.tick_params(axis="x", pad=4)
ax.set_ylabel("t $(1/\gamma)$")
ax.set_xlabel("n")

ax.set_box_aspect((4,4,2))
ax.yaxis.labelpad=10
ax.zaxis.labelpad=5
ax.xaxis.labelpad=10
fig.savefig('waveguide_occup.pdf', transparent=True)

==> enrstates.tex <==
import qutip as qt
import numpy as np

eps = 2 * np.pi
omega_c = 2 * np.pi
g = 0.1 * omega_c
gam = 0.01 * omega_c 
tlist = np.linspace(0,20,100)


N_cut = 2 #Number of Fock states to keep

psi0 = qt.basis(2, 0) & qt.basis(N_cut, 0) #initial state (qubit excitated)
sz = qt.sigmaz() & qt.qeye(N_cut)
sm = qt.sigmam() & qt.qeye(N_cut)
a = qt.qeye(2) & qt.destroy(N_cut)

H_JC = (
    0.5 * eps * sz + omega_c * a.dag() * a +
    g * (a * sm.dag() + a.dag() * sm)
) #Jaynes-Cummings Hamiltonian

c_ops = [np.sqrt(gam) * a]

result_JC = qt.mesolve(H_JC, psi0, tlist, c_ops, e_ops=[sz])


N_exc = 1 #Number of total excitations in truncated system
dims = [2, N_cut] #Original system dimensions (before ENR truncation)

psi0 = qt.enr_fock(dims, N_exc, [0, 0]) #Initial state in ENR space
sm, a = qt.enr_destroy(dims, N_exc) #operators in ENR space
sz = 2 * sm.dag() * sm - 1 

H_enr = (
    0.5 * eps * sz + omega_c * a.dag() * a +
    g * (sm.dag() * a + a.dag() * sm)
) #Jaynes-Cummings Hamiltonian

c_ops = [np.sqrt(gam) * a]

result_enr = qt.mesolve(H_enr, psi0, tlist, c_ops, e_ops=[sz]) 
    

==> heom_example.tex <==
# ---IMPORT SECTION---
from mpl_setup import BLUE, ORANGE, GREEN, PURPLE, GRAY, SKY_BLUE, VERMILLION
from qutip import Qobj, sigmaz, sigmax, brmesolve, sigmay
from qutip import sigmam, sigmap, mesolve, expect, basis
import numpy as np
from qutip.solver.heom import HEOMSolver, UnderDampedBath

import matplotlib.pyplot as plt
import mpmath as mp
from qutip import OhmicEnvironment, UnderDampedEnvironment, BosonicEnvironment
from qutip.core.environment import n_thermal

colors = [BLUE, ORANGE, GREEN, PURPLE, GRAY, SKY_BLUE, VERMILLION]
P11p = basis(2, 0) * basis(2, 0).dag()
P12p = basis(2, 0) * basis(2, 1).dag()

# -- FIRST EXAMPLE PARAMETERS ---

lam = 0.5
w0 = 1
gamma = 0.1
T = 0.5
t = np.linspace(0, 40, 1000)
rho0 = Qobj([[0, 0], [0, 1]])
Hsys = sigmax()/2 + 3*sigmaz()/4
Q = sigmaz()
env = UnderDampedEnvironment(lam=lam, gamma=gamma, T=T, w0=w0) #Create environment
bath = env.approximate("matsubara",Nk=5) #Approximate environment with Matsubara series

# -- SIMULATION --

# -- HEOM --
solver = HEOMSolver(Hsys, (bath, Q), max_depth=9)
result_h = solver.run(rho0, t)

# -- Lindblad manual --
all_energy, all_state = Hsys.eigenstates()
Nmax = len(all_state)
collapse_list = []
for i in range(Nmax):
    for j in range(Nmax):
        delE = (all_energy[j] - all_energy[i])
        if i!=j:
            rate = env.power_spectrum(delE) * (
                np.absolute(Q.matrix_element(all_state[i].dag(), all_state[j])) ** 2
            )

            if rate > 0:
                collapse_list.append(np.sqrt(rate) * all_state[i] * all_state[j].dag())
        else:
            rate = 2*env.power_spectrum(delE) * (
                np.absolute(Q.matrix_element(all_state[i].dag(), all_state[j])) ** 2
            )

            if rate > 0:
                collapse_list.append(np.sqrt(rate) * all_state[i] * all_state[j].dag())

result_lindblad = mesolve(Hsys, rho0, t, collapse_list)




# -- BLOCH-REDFIELD --
a_ops = [[Q, env]]
resultBR = brmesolve(Hsys, rho0, t, a_ops=a_ops, sec_cutoff=-1)


# -- DYNAMICS SIMULATION --
fig, ax = plt.subplots(1, 2, figsize=(13.6, 4.54))
ax[0].plot(lam*t, expect(P11p, result_h.states),
           color=colors[0], label='HEOMSolver',zorder=3)
ax[0].plot(lam*t, expect(P11p, result_lindblad.states),
            color=colors[1], label='mesolve')
ax[0].plot(lam*t, expect(P11p, resultBR.states),
           color=colors[2],linestyle=(0, (1, 1)), label='brmesolve')
ax[0].set_ylabel(r"$\rho_{11}$")
ax[0].set_xlabel(r"$\lambda t$")
ax[0].legend()
ax[1].plot(lam*t, expect(sigmap(), result_h.states),
           color=colors[0], label='HEOMSolver',zorder=3)
ax[1].plot(lam*t, expect(sigmap(), result_lindblad.states),
        color=colors[1], label='mesolve')
ax[1].plot(lam*t, expect(sigmap(), resultBR.states),
           color=colors[2],linestyle=(0, (1, 1)), label='brmesolve', markevery=10)

ax[1].set_ylabel(r"$Re(\rho_{12})$")
ax[1].set_xlabel(r"$\lambda t$")
ax[1].legend()
plt.savefig('./heom_qubit_underdamped.pdf')

# -- SECOND EXAMPLE PARAMETERS --
lam = 0.1
gamma = 5
T = 1

oh = OhmicEnvironment(T=T, alpha=lam, wc=gamma, s=1)

# -- FITTING PREDEFINED OHMIC CLASS--
w = np.linspace(0, 100, 2000) #Fitting range in frequency-domain
env_fs, _ = oh.approximate("sd",wlist=w, Nk=3, Nmax=3) #Fit spectral density


t = np.linspace(0, 10, 1000) #Fitting range in time-domain
env_fc, _ = oh.approximate("cf",tlist=t, Ni_max=5, Nr_max=4, 
                            target_rmse=None, maxfev=int(1e9)) #Fit correlation functions


# -- USING A USER DEFINED ENVIRONMENT --


def J(w, lam=lam, gamma=gamma):
    """ 
    Ohmic spectral density
    """
    return lam*w*np.exp(-abs(w)/gamma)


user_env = BosonicEnvironment.from_spectral_density(J, T=T, wMax=60)

user_env_sd, _ = user_env.approximate("sd",wlist=w, Nk=3, Nmax=3)

user_env_cf, _ = user_env.approximate("cf",tlist=t, Ni_max=5, Nr_max=4, target_rmse=None, maxfev=int(1e9))



# -- SOLVING DYNAMICS --
tlist = np.linspace(0, 10, 1000)
HEOM_corr_fit = HEOMSolver(Hsys, (env_fc, Q), max_depth=5)
result_corr = HEOM_corr_fit.run(rho0, tlist)

HEOM_spec_fit = HEOMSolver(Hsys, (env_fs, Q), max_depth=5)
result_spec = HEOM_spec_fit.run(rho0, tlist)


HEOM_fos = HEOMSolver(Hsys, (user_env_sd, Q),
                      max_depth=5)
result_fos = HEOM_fos.run(rho0, tlist)

HEOM_foc = HEOMSolver(Hsys, (user_env_cf, Q),
                      max_depth=5)
result_foc = HEOM_foc.run(rho0, tlist)

# -- OHMIC BATH DYNAMICS --
figfit, axfit = plt.subplots(1, 2, figsize=(13.6, 4.54))
full = oh.spectral_density(w)
axfit[0].plot(w, full, color=colors[0], label="Original")
j = 1
markers = ["-.", "--", "-."]
for i in [1, 10, 15]:
    bath_fs, fitinfo = oh.approximate("sd",wlist=w, Nmax=3, Nk=i)
    print(fitinfo["summary"])
    print("%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%")
    axfit[0].plot(w, bath_fs.spectral_density(
        w), linestyle=markers[j-1], color=colors[j], label=f"$N_k$={i}")
    axfit[1].plot(w, np.abs(full-bath_fs.spectral_density(w)),
                  markers[j-1], color=colors[j], label=f"$N_k$={i}")
    j += 1

axfit[0].legend()
axfit[1].legend()
axfit[0].set_ylabel(r"$J(\omega)$")
axfit[0].set_xlabel(r"$\omega$")
axfit[1].set_ylabel(r"$|J(\omega)-J_{approx}(\omega)|$")
axfit[1].set_xlabel(r"$\omega$")
plt.savefig('./heom_spec_k.pdf')

#figfit, axfit = plt.subplots(1, 2, figsize=(13.6, 4.54))
full = env_fs.correlation_function(t)
full_sd = env_fs.spectral_density(w)

# EXAMPLE OF COMPUTING APPROX CORRELATION FUNCTION
# -- FIRST EXAMPLE PARAMETERS ---

lam = 0.5
w0 = 1
gamma = 0.1
T = 0.5
env = UnderDampedEnvironment(lam=lam, gamma=gamma, T=T, w0=w0) #Exact environment
bath = env.approximate("matsubara",Nk=5) #Approximate environment
C = env.correlation_function(t) #Exact environment correlation functions
C2 = bath.correlation_function(t) #Approximate environment correlation functions

==> heom_transition.tex <==
#Warning, this example is very slow, it may take several hours to evaluate all data sets
import numpy as np
from matplotlib import pyplot as plt
from mpl_setup import BLUE, ORANGE, GREEN, PURPLE, GRAY, SKY_BLUE, VERMILLION
from qutip import *
from qutip.solver.heom import (
    HEOMSolver,
)
from qutip import BosonicEnvironment
colors = [BLUE, ORANGE, GREEN, PURPLE, GRAY, SKY_BLUE, VERMILLION]
eps = 0.1  # small system energy

Hsys = 0.5 * eps * sigmax()


def plot_result_expectations(result, color, label, m_op, axes=None, factor=1,
                             linestyle="solid"):
    """ Plot the expectation values of operators as functions of time.

        Each plot in plots consists of: (solver_result, measurement_operation,
        color, label).
    """
    if axes is None:
        fig, axes = plt.subplots(1, 1, sharex=True, figsize=(8, 8))
        fig_created = True
    else:
        fig = None
        fig_created = False

    # add kw arguments to each plot if missing
    exp = np.real(expect(result.states, m_op))
    axes.plot(np.array(result.times)*factor, exp, color=color, label=label,
              linestyle=linestyle)

    if fig_created:
        axes.legend(loc=0, fontsize=12)
        axes.set_xlabel("t", fontsize=28)

    return fig


# ALPHA
alphas = [0.1, 0.4, 0.6, 0.9, 1.2]
NCs = [8, 8, 8, 13, 13]

wc = 1

t = np.linspace(0, 80, 1000)
T = 0


def J(w, alpha=1):
    """ The Ohmic bath spectral density as a function
    of w (and the bath parameters). """
    return (np.pi/2) * w * alpha * 1 / (1+(w/wc)**2)**2


Q = sigmaz()
Ttot = 1200
# Times to solve for:
tlist = np.linspace(0, Ttot, 1000)
rho0 = basis(2, 0) * basis(2, 0).dag()

models = []
for i in range(len(alphas)):
    env = BosonicEnvironment.from_spectral_density(
        lambda w: J(w, alphas[i]), wMax=50, T=T)
    cfit, fitinfo = env.approximate(
       "cf", tlist=t, Ni_max=1, Nr_max=2, target_rmse=None, full_ansatz=True, maxfev=int(1e9)
    )
    
    print(fitinfo["summary"])
    options = {'nsteps': 15000, 'store_states': True,
                'rtol': 1e-7, 'atol': 1e-7}
    # Number of levels of the hierarchy to retain:
    NC = NCs[i]  # this is an importance covvergence parameter
    HEOMMats = HEOMSolver(Hsys, (cfit, Q), NC, options=options)
    resultMats = HEOMMats.run(rho0, tlist)
    models.append(resultMats)


fig, axes = plt.subplots(1, 1, sharex=True, figsize=(12, 5))
plt.axhline(y=0, label=r"$\langle \sigma_{z} \rangle$ =0" +
            " localized ", color=colors[len(alphas)], linestyle='--')
linestyles=['solid',"dashed","-.","dotted","solid"]

for k, i in enumerate(models):
    plot_result_expectations(
        i, colors[k], rf"$\alpha={alphas[k]} \quad N_c={NCs[k]}$",
        sigmaz(), axes=axes, factor=eps,linestyle=linestyles[k]
    )
# plt.xlim(0,1)
# axes.locator_param
axes.legend(loc=0, fontsize=18,bbox_to_anchor=(1.1, 1.05))
plt.ylabel(r"$\langle \sigma_{z}(t) \rangle$")
plt.xlabel(r"$\Delta t$")
fig.tight_layout()
plt.savefig('heom_transition.pdf')
# FOR The main text
def J(w, alpha=1):
    """ The Ohmic bath spectral density as a function
    of w (and the bath parameters). """
    return (np.pi/2) * w * alpha * 1 / (1+(w/wc)**2)**2

env = BosonicEnvironment.from_spectral_density(lambda w: J(w, alpha), wMax=50, T=T)

==> jax-countstats.tex <==
import qutip as qt
import jax
import jax.numpy as jnp
import qutip_jax  

from diffrax import Tsit5, PIDController as PID

options = {"method": "diffrax",
           "normalize_output": False,
           "stepsize_controller": PID(rtol=1e-7, atol=1e-7),
           "solver": Tsit5(scan_kind="bounded"),
           "progress_bar": False}


ed = 1 #Quantum dot energy
GammaL = 1 #Transport rate from left reservoir
GammaR = 1 #Transport rate to right reservoir

with jax.default_device(jax.devices("gpu")[0]):
    with qt.CoreOptions(default_dtype="jaxdia"):       
        d = qt.destroy(2)
        H = ed * d.dag() * d #Dot Hamiltonian
        c_op_L = jnp.sqrt(GammaL) * d.dag() #collapse operator for (input) left reservoir
        c_op_R = jnp.sqrt(GammaR) * d #collapse operator for (output) right reservoir

        L0 = (
            qt.liouvillian(H) + qt.lindblad_dissipator(c_op_L)
            - 0.5 * qt.spre(c_op_R.dag() * c_op_R)
            - 0.5 * qt.spost(c_op_R.dag() * c_op_R)
        ) #Liouvillian without Jump term to right reservoir
        #Jump term to right reservoir:
        L1 = qt.sprepost(c_op_R, c_op_R.dag()) 
        #Find steady state:
        rho0 = qt.steadystate(L0 + L1)
        
        
        def rhoz(t, z): #returns final system state (counting field z)
            L = L0 + jnp.exp(z) * L1  # jump term with counting-field 
            tlist = jnp.linspace(0, t, 50)     
            result = qt.mesolve(L, rho0, tlist, options=options)
            return result.final_state.tr()

        # first derivative
        drhozdz = jax.jacrev(rhoz, argnums=1) 
        # second derivative
        d2rhozdz = jax.jacfwd(drhozdz, argnums=1) 


tf = 100
Itest = GammaL * GammaR / (GammaL + GammaR)
print("Analytic current", Itest)
print("Numerical current", drhozdz(tf, 0.) / tf)
print("Analytical shot noise (2nd cumulant)",
      Itest * (1 - 2 * GammaL * GammaR / (GammaL + GammaR)**2))
print("Numerical shot noise (2nd cumulant)",
      (d2rhozdz(tf, 0.) - drhozdz(tf, 0.)**2) / tf)

?\pythonoutput?Analytic current 0.5
?\pythonoutput?Numerical current 0.4999
?\pythonoutput?Analytical shot noise (2nd cumulant) 0.25
?\pythonoutput?Numerical shot noise (2nd cumulant) 0.25125


import jax
import jax.numpy as jnp
import qutip
import qutip_jax

# Set JAX backend for QuTiP
qutip_jax.set_as_default()

# Define time-dependent driving function
@jax.jit
def driving_coeff(t, omega):
    return jnp.cos(omega * t)

# Define the system Hamiltonian
def setup_system(omega):
    H_0 = qutip.sigmaz() #Hamiltonian (time-independent)
    H_1 = qutip.sigmax()  #Hamiltonian (driven part, time-dependent)
    H = [H_0, [H_1, driving_coeff]]  #Total Hamiltonian (QobjEvo)
    return H

gamma = 0.1  # Dissipation rate
c_ops = [jnp.sqrt(gamma) * qutip.sigmam()]
psi0 = qutip.basis(2, 0) #Initial state

tlist = jnp.linspace(0.0, 10.0, 100) #time steps

e_ops = [qutip.projection(2, 1, 1)]

# Objective function: simulate and return the population of the excited state at final time
def f(omega):
    H = setup_system(omega)
    result = qutip.mcsolve(H, psi0, tlist, c_ops, e_ops, ntraj=100, args = {"omega": omega})
    return result.expect[0][-1]  

# Compute gradient of the excited-state population w.r.t. omega
grad_f = jax.grad(f)(2.0)


==> jax-mesolve.tex <==
import qutip as qt

import jax
import jax.numpy as jnp
import qutip_jax  # noqa: F401

print(qt.qeye(3, dtype='jax').dtype.__name__)
?\pythonoutput?JaxArray

print(qt.qeye(3, dtype='jaxdia').dtype.__name__)
?\pythonoutput?JaxDia

def Ising_solve(N, g0, J0, gamma, tlist, options, data_type='CSR'):
    # N  : number of spins
    # g0 : splitting
    # J0 : couplings
    with qt.CoreOptions(default_dtype=data_type):

        #Setup operators for individual qubits
        sx_list, sy_list, sz_list = [], [], []
        for i in range(N):
            op_list = [qt.qeye(2)] * N
            op_list[i] = qt.sigmax()
            sx_list.append(qt.tensor(op_list))
            op_list[i] = qt.sigmay()
            sy_list.append(qt.tensor(op_list))
            op_list[i] = qt.sigmaz()
            sz_list.append(qt.tensor(op_list))

        # Hamiltonian - Energy splitting terms
        H = 0.
        for i in range(N):
            H += g0 * sz_list[i]

        # Interaction terms
        for n in range(N - 1):
            H += -J0 * sx_list[n] * sx_list[n + 1]

        # Collapse operator acting locally on single spin
        c_ops = [gamma * sx_list[N-1]]

        # Initial state
        state_list = [qt.basis(2, 1)] * (N-1)
        state_list.append(qt.basis(2, 0))
        psi0 = qt.tensor(state_list)

        result = qt.mesolve(H, psi0, tlist, c_ops, e_ops=sz_list, options=options)
        return result, result.expect[-1]


from diffrax import PIDController, Tsit5

with jax.default_device(jax.devices("gpu")[0]):
    # System parameters
    N = 4 #number of spins
    g0 = 1 #energy splitting of spins
    J0 = 1.4 #spin-spin coupling
    gamma = 0.1 #dissipation rate

    # Simulation parameters
    tlist = jnp.linspace(0, 5, 100) #times steps
    options = {
        "normalize_output": False,
        "store_states": True,
        "method": "diffrax",
        "stepsize_controller": PIDController(rtol=qt.settings.core['rtol'],
                                             atol=qt.settings.core['atol']),
        "solver": Tsit5()
    }

    result_ising, sz1 = Ising_solve(N, g0, J0, gamma, tlist, options, data_type='jaxdia')



# Use JAX as the backend
qutip_jax.set_as_default()


qutip_jax.set_as_default(revert=True)

==> mcsolve.tex <==
import qutip as qt
import numpy as np

ntraj = 100
epsilon1 = 1.0
epsilon2 = 1.0
g = 0.1

sx1 = qt.sigmax() & qt.qeye(2)
sx2 = qt.qeye(2) & qt.sigmax()
sz1 = qt.sigmaz() & qt.qeye(2)
sz2 = qt.qeye(2) & qt.sigmaz()

H = (epsilon1 / 2) * sz1 + (epsilon2 / 2) * sz2 + g * sx1 * sx2

sm1 = qt.sigmam() & qt.qeye(2)
sm2 = qt.qeye(2) & qt.sigmam()
gam = 0.1  # dissipation rate
c_ops = [np.sqrt(gam) * sm1, np.sqrt(gam) * sm2]
psi0 = qt.basis(2, 0) & qt.basis(2, 1)
tlist = np.linspace(0, 40, 100)

result_mc = qt.mcsolve(H, psi0, tlist, c_ops, e_ops=[sz1, sz2], ntraj=ntraj,
                       options={"map": "parallel", "keep_runs_results": True})
result_me = qt.mesolve(H, psi0, tlist, c_ops, e_ops=[sz1, sz2])

import matplotlib.pyplot as plt
from mpl_setup import * 
plt.figure()
plt.plot(tlist, result_me.expect[0],'-', label=r'mesolve')
plt.plot(tlist, result_mc.average_expect[0],'--',alpha=1,label=r'mcsolve average')
plt.fill_between(
    tlist,
    (result_mc.average_expect[0] - result_mc.std_expect[0] / np.sqrt(ntraj)) ,
    (result_mc.average_expect[0] + result_mc.std_expect[0] / np.sqrt(ntraj)),
    alpha=0.5, color="ORANGE"
)
plt.plot(tlist, result_mc.runs_expect[0][4],'-.',label=r'mcsolve 1 run')
plt.plot(tlist, result_mc.runs_expect[0][7],':',label=r'mcsolve 1 run')

plt.xlabel('Time', fontsize=18)
plt.ylabel(r'$\langle \sigma_z^{(1)} \rangle$', fontsize=18)
plt.legend()
plt.savefig("mcsolve.pdf")
plt.show()


==> mesolve.tex <==
import qutip as qt
import numpy as np

epsilon1 = 1.0
epsilon2 = 1.0
g = 0.1

sx1 = qt.sigmax() & qt.qeye(2) 
sx2 = qt.qeye(2) & qt.sigmax()
sz1 = qt.sigmaz() & qt.qeye(2)
sz2 = qt.qeye(2) & qt.sigmaz()

H = (epsilon1 / 2) * sz1 + (epsilon2 / 2) * sz2 + g * sx1 * sx2

sm1 = qt.sigmam() & qt.qeye(2)
sm2 = qt.qeye(2) & qt.sigmam()
gam = 0.1  # dissipation rate
c_ops = [np.sqrt(gam) * sm1, np.sqrt(gam) * sm2] #list of collapse operators for solver
psi0 = qt.basis(2, 0) & qt.basis(2, 1) #initial state (qubit 1 excitated)
tlist = np.linspace(0, 40, 100) #time steps

result_me = qt.mesolve(H, psi0, tlist, c_ops, e_ops=[sz1, sz2]) #run mesolve
print(result_me)
?\pythonoutput?<Result
?\pythonoutput?  Solver: mesolve
?\pythonoutput?  Solver stats:
?\pythonoutput?    method: 'scipy zvode adams'
?\pythonoutput?    init time: 8.153915405273438e-05
?\pythonoutput?    preparation time: 0.00011157989501953125
?\pythonoutput?    run time: 0.0024967193603515625
?\pythonoutput?    solver: 'Master Equation Evolution'
?\pythonoutput?    num_collapse: 2
?\pythonoutput?  Time interval: [0.0, 40.0] (100 steps)
?\pythonoutput?  Number of e_ops: 2
?\pythonoutput?  State not saved.
?\pythonoutput?>

lindbladian = -1.0j * (qt.spre(H) - qt.spost(H)) #Hamiltonian term
for c in c_ops:
    lindbladian += (
        qt.sprepost(c, c.dag()) - 0.5 * (qt.spre(c.dag() * c) + qt.spost(c.dag() * c))
    ) #Manual construction of Lindblad

result_me2 = qt.mesolve(lindbladian, psi0, tlist,  [], e_ops = [sz1, sz2])


def power_spectrum(w):
    if w >= 0:
        return gam #flat power spectrum
    else:
        return 0 #Zero temperature: only has support on positive frequencies 

all_energy, all_state = H.eigenstates() #get eigenstates (ES)
Nmax = len(all_state)
collapse_list = []
for i in range(Nmax):
    for j in range(Nmax):
        delE = (all_energy[j] - all_energy[i]) #energy splitting between ES
        rate = power_spectrum(delE) * (
            np.absolute(sx1.matrix_element(all_state[i].dag(), all_state[j])) ** 2
            + np.absolute(sx2.matrix_element(all_state[i].dag(), all_state[j])) ** 2
        ) #Rates for both qubits 
        if rate > 0: #add to collapse operator list
            collapse_list.append(np.sqrt(rate) * all_state[i] * all_state[j].dag())

tlist_long = np.linspace(0, 1000, 100) #time steps
result_me_global = qt.mesolve(H, psi0, tlist_long, collapse_list) #run mesolve 
fidelity = qt.fidelity(result_me_global.states[-1], all_state[0] @ all_state[0].dag())
print(f"Fidelity with ground-state: {fidelity:.6f}") #compare final state with ground state
?\pythonoutput?Fidelity with ground-state: 1.000000




def power_spectrum(w):
    if w >= 0: #Zero-temperature, only has positive-frequency support
        return gam
    else:
        return 0

result_BR = qt.brmesolve(H, psi0, tlist, e_ops=[sz1, sz2],
                         a_ops=[[sx1, power_spectrum], [sx2, power_spectrum]])

# repeat mesolve simulation with different tlist
result_me_global = qt.mesolve(H, psi0, tlist, collapse_list, e_ops = [sz1, sz2])

import matplotlib.pyplot as plt
from mpl_setup import * 
plt.figure()
plt.plot(tlist, result_me.expect[0], label=r'Local Lindblad')
plt.plot(tlist, result_me_global.expect[0],'--',label=r'Dressed Lindblad')
plt.plot(tlist, result_BR.expect[0],':',label=r'Bloch-Redfield')
plt.xlabel('Time', fontsize=18)
plt.ylabel(r'$\langle \sigma_z^{(1)} \rangle$', fontsize=18)
plt.legend()
plt.text(10,0.7,"(a)", fontsize=18)
#plt.savefig("mesolve-fig1.pdf")
plt.show()


==> mesolvedriven.tex <==
import numpy as np
import qutip as qt
from qutip.solver.heom import HEOMSolver, BosonicBath
from qutip import UnderDampedEnvironment, QobjEvo
import matplotlib.pyplot as plt
from mpl_setup import *


############ Normal driven qubit, time-dependent example 1 for paper ##########


# Hamiltonian parameters
Delta = 2 * np.pi  # qubit splitting
omega_d = Delta  # drive frequency
A = 0.01 * Delta  # drive amplitude

# Driving field


def f(t):
    return np.sin(omega_d * t)


# Time-dependent Hamiltonian
H0 = Delta / 2.0 * qt.sigmaz()
H1 = [A / 2.0 * qt.sigmax(), f]
H = [H0, H1]

# Bath parameters
gamma = 0.005 * Delta / (2 * np.pi)  # dissipation strength
temp = 0  # temperature

# Simulation parameters
psi0 = qt.basis(2, 0)  # initial state
e_ops = [qt.sigmaz()]

T = 2 * np.pi / omega_d  # period length
tlist = np.linspace(0, 1000 * T, 500)


# --- mesolve ---

c_ops_me = [np.sqrt(gamma) * qt.sigmam()]
me_result = qt.mesolve(H, psi0, tlist, c_ops=c_ops_me, e_ops=e_ops)


# --- mesolve, RWA ---

c_ops_me_RWA = [np.sqrt(gamma) * qt.sigmam()]
H_RWA = (Delta - omega_d) * 0.5 * qt.sigmaz() + A / 4 * qt.sigmax()
me_result_RWA = qt.mesolve(H_RWA, psi0, tlist, c_ops=c_ops_me_RWA, e_ops=e_ops)


# --- HEOM ---

# Numerical parameters
max_depth = 4  # number of hierarchy levels
fit_times = np.linspace(0, 25, 1000)  # range for correlation function fit

# Emulate flat spectral density with an underdamped spectral density
wsamp = 2 * np.pi
w0 = 5 * 2 * np.pi
gamma_heom = 1.9 * w0
Gamma = gamma_heom / 2

Omega = np.sqrt(w0**2 - Gamma**2)
lambd = np.sqrt(
    0.5 * gamma / (gamma_heom * wsamp) *
    ((w0 ** 2 - wsamp ** 2) ** 2 + (gamma_heom ** 2) * ((wsamp) ** 2))
)
# Create Environment
bath = UnderDampedEnvironment(lam=lambd, w0=w0, gamma=gamma_heom, T=0)

# To handle zero-temperature underdamped bath, fit its correlation function
exp_bath, fit_info = bath.approximate("cf",fit_times, Ni_max=1, Nr_max=3, target_rmse=None)
print(fit_info['summary'])



# # Do simulation
HEOM_corr_fit = HEOMSolver(QobjEvo(H), (exp_bath, qt.sigmax()), max_depth=max_depth,
                    options={'nsteps': 15000, 'rtol': 1e-12, 'atol': 1e-12})
results_corr_fit = HEOM_corr_fit.run(psi0 * psi0.dag(), tlist, e_ops=e_ops)

# --- brmesolve ---

# Bose einstein distribution
def nth(w): # Bose einstein distribution
    if temp > 0:
        return 1 / (np.exp(w / temp) - 1)
    else:
        return 0

def power_spectrum(w):# Power spectrum
    if w > 0: #Influences emission
        return gamma * (nth(w) + 1)
    elif w == 0:
        return 0
    else: #Influences absorption
        return gamma * nth(-w)

a_ops = [[qt.sigmax(), power_spectrum]] #system operator which couples to bath, and 
                                        #bath power spectrum are needed
brme_result = qt.brmesolve(H, psi0, tlist, a_ops=a_ops, e_ops=e_ops, sec_cutoff=-1)


# --- Plots ---

plt.figure()

plt.plot(tlist, me_result.expect[0], '-', label=r'mesolve (time-dep)')
plt.plot(tlist, me_result_RWA.expect[0], '-.', label=r'mesolve (rwa)')
plt.plot(tlist, results_corr_fit.expect[0], '--', label=r'heomsolve')
plt.plot(tlist, brme_result.expect[0], ':', linewidth=6, label=r'brmesolve')

plt.xlabel(r'$t\, /\, \Delta^{-1}$', fontsize=18)
plt.ylabel(r'$\langle \sigma_z \rangle$', fontsize=18)
plt.legend()
plt.text(200, 0.7, "(a)", fontsize=18)

plt.savefig("mesolve_driven_1.pdf")


############ Frequency modulation, Example 2 ############

# hamiltonian parameters
omega_d = 0.05 * Delta  # drive frequency
A = Delta  # drive amplitude

# driving field


def f(t):
    return np.sin(omega_d * t)


H0 = [A / 2.0 * qt.sigmaz(), f]
H = [H0]

# bath parameters
gamma = 0.05 * Delta / (2 * np.pi)  # dissipation strength

# simulation parameters
psi0 = qt.basis(2, 0)  # initial state
e_ops = [qt.sigmaz()]

T = 2 * np.pi / omega_d  # period length
tlist = np.linspace(0, 2 * T, 400)

# --- HEOM ---

wsamp = 2 * np.pi
w0 = 5 * 2 * np.pi

gamma_heom = 1.9 * w0
# gamma = 1.5 * w0


lambd = np.sqrt(
    0.5 * gamma *
    ((w0 ** 2 - wsamp ** 2) ** 2 + (gamma_heom ** 2) * ((wsamp) ** 2)) /
    (gamma_heom * wsamp))


# --- mesolve ---

c_ops_me = [np.sqrt(gamma) * qt.sigmam()]
me_result = qt.mesolve(H, psi0, tlist, c_ops=c_ops_me, e_ops=e_ops)


# --- mesolve, RWA ---

c_ops_me_RWA = [np.sqrt(gamma) * qt.sigmam()]
H_RWA = (Delta - omega_d) * 0.5 * qt.sigmaz() + A / 4 * qt.sigmax()
me_result_RWA = qt.mesolve(H_RWA, psi0, tlist, c_ops=c_ops_me_RWA, e_ops=e_ops)


# --- HEOM ---

# Create Environment
bath = UnderDampedEnvironment(lam=lambd, w0=w0, gamma=gamma_heom, T=0)
fit_times = np.linspace(0, 5, 1000)  # range for correlation function fit

# To handle zero-temperature underdamped, fit its correlation function

exp_bath, fit_info = bath.approximate("cf",fit_times, Ni_max=1, Nr_max=2, target_rmse=None)
print(fit_info['summary'])




HEOM_corr_fit = HEOMSolver(QobjEvo(H), (exp_bath, qt.sigmax()), max_depth=max_depth,
                           options={"nsteps": 15000, "rtol": 1e-12, "atol": 1e-12})
results_corr_fit = HEOM_corr_fit.run(psi0 * psi0.dag(), tlist, e_ops=e_ops)


# --- brmesolve ---

a_ops = [[qt.sigmax(), exp_bath]]
brme_result = qt.brmesolve(H, psi0, tlist, a_ops=a_ops, e_ops=e_ops)

a_ops = [[qt.sigmax(), power_spectrum]]
brme_result2 = qt.brmesolve(H, psi0, tlist, a_ops=a_ops, e_ops=e_ops)


# --- Plots ---

plt.figure()

plt.plot(tlist, me_result.expect[0], '-', label=r'mesolve')
plt.plot(tlist, results_corr_fit.expect[0], '--', label=r'heomsolve')
plt.plot(
    tlist, brme_result.expect[0],
    ':', linewidth=6, label=r'brmesolve non-flat')
plt.plot(tlist, brme_result2.expect[0], ':', linewidth=6, label=r'brmesolve')

plt.xlabel(r'$t\, /\, \Delta^{-1}$', fontsize=18)
plt.ylabel(r'$\langle \sigma_z \rangle$', fontsize=18)
plt.legend()
plt.text(8, 0.7, "(b)", fontsize=18)

plt.savefig("mesolve_driven_2.pdf")

############ Alternative ways of specifying time dependence ############

f = f"sin({omega_d} * t)"

f = np.sin(omega_d * tlist)

==> nm_mcsolve_example.tex <==
from mpl_setup import ORANGE, BLUE, GREEN, GRAY

import numpy as np
from scipy.interpolate import CubicSpline
from scipy.optimize import root_scalar
import qutip as qt
import matplotlib.pyplot as plt



# ----- SYSTEM PARAMETERS -----

# --- Numerics ---

tlist = np.linspace(0, 5, 500)

# --- Initial state ---

alphap = 1 / np.sqrt(2)
alpham = np.sqrt(1 - alphap**2)

initial_state = alphap * qt.basis(2, 0) + alpham * qt.basis(2, 1)

# --- Constants ---

gamma0 = 1
lamb = 0.3 * gamma0
Delta = 8 * lamb

# --- Derived quantities ---

delta = np.sqrt((lamb - 1j * Delta)**2 - 2 * gamma0 * lamb)
deltaR = np.real(delta)
deltaI = np.imag(delta)
deltaSq = deltaR**2 + deltaI**2

def TCL_params(t):
    common_factor = 2 * gamma0 * lamb / (
        (lamb**2 + Delta**2 - deltaSq) * np.cos(deltaI * t)
        - (lamb**2 + Delta**2 + deltaSq) * np.cosh(deltaR * t)
        - 2 * (Delta * deltaR + lamb * deltaI) * np.sin(deltaI * t)
        + 2 * (Delta * deltaI - lamb * deltaR) * np.sinh(deltaR * t)
    )
    gamma = common_factor * (
        lamb * np.cos(deltaI * t) - lamb * np.cosh(deltaR * t)
        - deltaI * np.sin(deltaI * t) - deltaR * np.sinh(deltaR * t)
    )
    A = common_factor * (
        Delta * np.cos(deltaI * t) - Delta * np.cosh(deltaR * t)
        - deltaR * np.sin(deltaI * t) + deltaI * np.sinh(deltaR * t)
    )
    return gamma, A

# --- Interpolate TCL params for better performance ---

_gamma = np.zeros_like(tlist)
_A = np.zeros_like(tlist)
for i in range(len(tlist)):
    _gamma[i], _A[i] = TCL_params(tlist[i])

gamma = CubicSpline(tlist, np.complex128(_gamma))
A = CubicSpline(tlist, np.complex128(_A))



# ----- MESOLVE -----

H = qt.sigmap() * qt.sigmam() / 2
unitary_gen = qt.liouvillian(H)
dissipator = qt.lindblad_dissipator(qt.sigmam())

me_solution = qt.mesolve([[unitary_gen, A], [dissipator, gamma]], initial_state, tlist)



# ----- NM_MCSOLVE -----

mc_solution = qt.nm_mcsolve([[H, A]], initial_state, tlist,
                            ops_and_rates=[(qt.sigmam(), gamma)],
                            ntraj=1_000, options={'map': 'parallel'}, seeds=0)



# ----- HEOM -----

# --- Schroedinger picture ---

# We are not in the interaction picture any more
# Choose, omega_c, omega_0 so that RWA is good
omega_c = 100
omega_0 = omega_c + Delta

H = omega_0 * qt.sigmap() * qt.sigmam()
Q = qt.sigmap() + qt.sigmam()

# --- Construct HEOM rhs ---

ck_real = [gamma0 * lamb / 4] * 2
vk_real = [lamb - 1j * omega_c, lamb + 1j * omega_c]
ck_imag = np.array([1j, -1j]) * gamma0 * lamb / 4
vk_imag = vk_real

heom_bath = qt.heom.BosonicBath(Q, ck_real, vk_real, ck_imag, vk_imag)

# --- Go ---

heom_solution = qt.heom.heomsolve(H, heom_bath, 10, qt.ket2dm(initial_state), tlist)

# --- Transform to interaction picture ---

Us = [(-1j * H * t).expm() for t in tlist]
heom_states = [U * state * U.dag() for (U, state) in zip(Us, heom_solution.states)]



# ----- BLOCH REDFIELD -----

def power_spectrum(w):
    return gamma0 * lamb**2 / ((omega_c - w)**2 + lamb**2)

br_solution = qt.brmesolve(H, initial_state, tlist, a_ops=[(qt.sigmax(), power_spectrum)])
br_states = [U * state * U.dag() for (U, state) in zip(Us, br_solution.states)]



# ----- PLOTS -----

# zeroes of gamma(t)
root1 = root_scalar(lambda t: TCL_params(t)[0], method='bisect', bracket=(1, 2)).root
root2 = root_scalar(lambda t: TCL_params(t)[0], method='bisect', bracket=(2, 3)).root
root3 = root_scalar(lambda t: TCL_params(t)[0], method='bisect', bracket=(3, 4)).root
root4 = root_scalar(lambda t: TCL_params(t)[0], method='bisect', bracket=(4, 5)).root

fig, ax = plt.subplots(1, 3, figsize=(13.6, 4.54))

# --- rho_11 ---

projector = (qt.sigmaz() + qt.qeye(2)) / 2
ax[0].plot(tlist, qt.expect(projector, me_solution.states),
           '-', color=ORANGE, label=r'mesolve')
ax[0].plot(tlist[::10], qt.expect(projector, mc_solution.states[::10]),
           'x', color=BLUE, label=r'nm_mcsolve')
ax[0].plot(tlist, qt.expect(projector, heom_states),
           '--', color=GREEN, label=r'heomsolve')
ax[0].plot(tlist, qt.expect(projector, br_states),
           '-.', color=GRAY, label=r'brmesolve')

ax[0].set_xlabel(r'$t\, /\, \lambda^{-1}$', fontsize=18)
ax[0].set_xlim((-0.2, 5.2))
ax[0].set_xticks([0, 2.5, 5], labels=[r'$0$', r'$2.5$', r'$5$'])
ax[0].set_title(r'$\rho_{11}$', fontsize=18, pad=10)
ax[0].set_ylim((0.4376, 0.5024))
ax[0].set_yticks([0.44, 0.46, 0.48, 0.5], labels=[r'$0.44$', r'$0.46$', r'$0.48$', r'$0.50$'])

ax[0].axvspan(root1, root2, color=GRAY, alpha=0.08, zorder=0)
ax[0].axvspan(root3, root4, color=GRAY, alpha=0.08, zorder=0)

ax[0].legend(frameon=1, framealpha=1)

# --- | rho_01 |^2 ---

me_x = qt.expect(qt.sigmax(), me_solution.states)
mc_x = qt.expect(qt.sigmax(), mc_solution.states[::10])
heom_x = qt.expect(qt.sigmax(), heom_states)
br_x = qt.expect(qt.sigmax(), br_states)

me_y = qt.expect(qt.sigmay(), me_solution.states)
mc_y = qt.expect(qt.sigmay(), mc_solution.states[::10])
heom_y = qt.expect(qt.sigmay(), heom_states)
br_y = qt.expect(qt.sigmay(), br_states)

# The HEOM result oscillates with a very small amplitude that isn't
# visible in the plot but makes the dashing wonky. Let's smoothen.
heom_plot = heom_x * heom_x + heom_y * heom_y
heom_plot = np.convolve(heom_plot, np.array([1 / 11] * 11), mode='valid')
heom_tlist = tlist[5 : -5]

ax[1].plot(tlist, me_x * me_x + me_y * me_y,
           '-', color=ORANGE, label=r'mesolve')
ax[1].plot(tlist[::10], mc_x * mc_x + mc_y * mc_y,
           'x', color=BLUE, label=r'nm_mcsolve')
ax[1].plot(heom_tlist, heom_plot,
           '--', color=GREEN, label=r'heomsolve')
ax[1].plot(tlist, br_x * br_x + br_y * br_y,
           '-.', color=GRAY, label=r'brmesolve')

ax[1].set_xlabel(r'$t\, /\, \lambda^{-1}$', fontsize=18)
ax[1].set_xlim((-0.2, 5.2))
ax[1].set_xticks([0, 2.5, 5], labels=[r'$0$', r'$2.5$', r'$5$'])
ax[1].set_title(r'$| \rho_{01} |^2$', fontsize=18, pad=10)
ax[1].set_ylim((0.8752, 1.0048))
ax[1].set_yticks([0.88, 0.9, 0.92, 0.94, 0.96, 0.98, 1],
                 labels=[r'$0.88$', r'$0.90$', r'$0.92$', r'$0.94$', r'$0.96$', r'$0.98$', r'$1$'])

ax[1].axvspan(root1, root2, color=GRAY, alpha=0.08, zorder=0)
ax[1].axvspan(root3, root4, color=GRAY, alpha=0.08, zorder=0)

ax[1].legend(frameon=1, framealpha=1)

# --- Martingale ---

ax[2].plot(tlist, np.zeros_like(tlist), '-', color=ORANGE, label=r'Zero')
ax[2].plot(tlist[::10], 1000 * (mc_solution.trace[::10] - 1), 'x', color=BLUE, label=r'nm_mcsolve')

ax[2].set_xlabel(r'$t\, /\, \lambda^{-1}$', fontsize=18)
ax[2].set_xlim((-0.2, 5.2))
ax[2].set_xticks([0, 2.5, 5], labels=[r'$0$', r'$2.5$', r'$5$'])
ax[2].set_title(r'$(\mu - 1)\, /\, 10^{-3}$', fontsize=18, pad=10)
ax[2].set_ylim((-5.8, 15.8))
ax[2].set_yticks([-5, 0, 5, 10, 15])

ax[2].axvspan(root1, root2, color=GRAY, alpha=0.08, zorder=0)
ax[2].axvspan(root3, root4, color=GRAY, alpha=0.08, zorder=0)

ax[2].legend(frameon=1, framealpha=1)

plt.savefig('./nm_mcsolve_figure.pdf')



exit()
# ----- FORMATTING FOR PAPER -----

H = qt.sigmap() * qt.sigmam() / 2 #Hamiltonian 
initial_state = (qt.basis(2, 0) + qt.basis(2, 1)).unit()  #initial state
tlist = np.linspace(0, 5, 500) #time steps



unitary_gen = qt.liouvillian(H) #Hamiltonian term
dissipator = qt.lindblad_dissipator(qt.sigmam()) #Lindblad term (no rate included)
me_solution = qt.mesolve([[unitary_gen, A], [dissipator, gamma]], initial_state, tlist)



mc_solution = qt.nm_mcsolve([[H, A]], initial_state, tlist,
                            ops_and_rates=[(qt.sigmam(), gamma)],
                            ntraj=1_000, options={'map': 'parallel'})



H = omega_0 * qt.sigmap() * qt.sigmam() #Hamiltonian
Q = qt.sigmap() + qt.sigmam() #system operator which couples to the bath



ck_real = [gamma0 * lamb / 4] * 2 #Real term prefactors
vk_real = [lamb - 1j * omega_c, lamb + 1j * omega_c] #Real term exponents
ck_imag = np.array([1j, -1j]) * gamma0 * lamb / 4 #Imag term prefactors
vk_imag = vk_real #Imag term exponents

heom_bath = qt.heom.BosonicBath(Q, ck_real, vk_real, ck_imag, vk_imag) #create bath
heom_solution = qt.heom.heomsolve(H, heom_bath, 10, qt.ket2dm(initial_state), tlist)



def power_spectrum(w):
    return gamma0 * lamb**2 / ((omega_c - w)**2 + lamb**2)

br_solution = qt.brmesolve(H, initial_state, tlist, a_ops=[(qt.sigmax(), power_spectrum)])



Us = [(-1j * H * t).expm() for t in tlist] #Transformation operator
heom_states = [U * state * U.dag() for (U, state) in zip(Us, heom_solution.states)]
br_states = [U * state * U.dag() for (U, state) in zip(Us, br_solution.states)]

==> p_Floquet_speed_test.tex <==
import matplotlib.pyplot as plt
import mpl_setup
import numpy as np

import qutip as qt
import time

PI = np.pi


## ====================================================
## Defining the system and initial states
## ====================================================

# ----------------------------------------
# Defining the Hamiltonian
# ----------------------------------------
delta = 0.2 * 2*PI
epsilon = 1.0 * 2*PI
A = 2.5 * 2*PI
omega = 1.0 * 2*PI
T = 2*PI / omega

# Initial condition
psi0 = qt.basis(2, 0)

# Hamiltonian
H0 = -1 / 2 * (epsilon * qt.sigmaz() + delta * qt.sigmax()) #Hamiltonian (static)
H1 = A / 2 * qt.sigmax() #Hamiltonian (driven part)
args = {'w': omega}
H = [H0, [H1, lambda t, w: np.sin(w * t)]] #Creates a QobjEvo Hamiltonian

# Numerical parameters
dt = .01
N_T = 10  # Number of periods
tlist = np.arange(0.0, N_T * T, dt)  # time-list


# ======================================================
# Initialization of arrays
# ======================================================
computational_time_floquet = np.zeros_like(tlist)
computational_time_sesolve = np.zeros_like(tlist)

expect_floquet = np.zeros_like(tlist)
expect_sesolve = np.zeros_like(tlist)


# ======================================================
# Starting simulation
# ======================================================
for n, t in enumerate(tlist):
    # --------------------------------
    # Floquet basis
    # --------------------------------
    tic_f = time.perf_counter()
    floquetbasis = qt.FloquetBasis(H, T, args)
    # Decomposing inital state into Floquet modes
    f_coeff = floquetbasis.to_floquet_basis(psi0)
    # Obtain evolved state in the original basis
    psi_t = floquetbasis.from_floquet_basis(f_coeff, t)
    p_ex = qt.expect(qt.sigmaz(), psi_t)
    toc_f = time.perf_counter()

    # Saving data
    computational_time_floquet[n] = toc_f - tic_f
    expect_floquet[n] = p_ex

    # --------------------------------
    # sesolve
    # --------------------------------
    tic_f = time.perf_counter()
    p_ex_ref = qt.sesolve(H, psi0, tlist[:n + 1], e_ops=[qt.sigmaz()], args=args).expect[0]
    toc_f = time.perf_counter()
    # Saving data
    computational_time_sesolve[n] = toc_f - tic_f
    expect_sesolve[n] = p_ex_ref[-1]


# ======================================================
# Plotting results
# ======================================================
sty = ["-", "--"]
fig, axs = plt.subplots(1, 2, figsize=(13.6, 4.5))
ax = axs[0]
ax.plot(tlist / T, computational_time_floquet, sty[0])
ax.plot(tlist / T, computational_time_sesolve, sty[1])

axs[0].set_yscale("log")
axs[0].set_yticks(np.logspace(-3, -1, 3))
axs[1].plot(tlist / T, np.real(expect_floquet), sty[0], lw='3.5')
axs[1].plot(tlist / T, np.real(expect_sesolve), sty[1], lw='3.5')

axs[0].set_xlabel(r'$t \, / \, T$')
axs[1].set_xlabel(r'$t \, / \, T$')
ax.set_ylabel(r'Computational Time [$s$]')
axs[1].set_ylabel(r'$\langle \sigma_z \rangle$')
ax.legend((r"Floquet", r"sesolve"), frameon=False)
xticks = np.rint(np.linspace(0, N_T, N_T + 1, endpoint=True))
axs[0].set_xticks(xticks)
axs[0].set_xlim([0, N_T])
axs[1].set_xticks(xticks)
axs[1].set_xlim([0, N_T])
axs[0].text(-.15, 1.05, r'(a)', transform=axs[0].transAxes)
axs[1].text(-.15, 1.05, r'(b)', transform=axs[1].transAxes)

fig.show()
fig.savefig('./floquet_speed_test.pdf')



exit()
# For formatting in paper, stripped leading whitespace

floquetbasis = qt.FloquetBasis(H, T, args)
# Decomposing inital state into Floquet modes
f_coeff = floquetbasis.to_floquet_basis(psi0)
# Obtain evolved state in the original basis
psi_t = floquetbasis.from_floquet_basis(f_coeff, t)

==> p_Ising_with_drive_Floquet.tex <==
import matplotlib.pyplot as plt
import mpl_setup
import numpy as np

import qutip as qt
import time

PI = np.pi


## ====================================================
#                    Input Parameters
## ====================================================

# ----------------------------------------
# Defining the Hamiltonian constants
# ----------------------------------------
# Number of spins
N = 4
# Energy-splitting
g0 = 1
# Coupling strength
J0 = 1.4
# Drive strength
A = 1.  # Drive norm.

# Drive frequency and period
omega = 1.0 * 2 * PI  # drive angular frequency
T = 2*PI / omega  # Drive period

# ---------------------------------
# Numerical sampling
# ---------------------------------
N_T = 10
dt = 0.01
tlist = np.arange(0, N_T * T, dt)
tlist_0 = np.arange(0, T, dt)  # One period tlist


# ======================================================
# Creating Hamiltonian
# ======================================================

def setup_Ising_drive(N, g0, J0, A, omega, data_type='CSR'):
    """
    # N    : number of spins
    # g0   : splitting,
    # J0   : couplings
    # A    : drive amplitude
    # omega: drive frequency
    """
    with qt.CoreOptions(default_dtype=data_type):

        sx_list, sy_list, sz_list = [], [], []
        for i in range(N):
            op_list = [qt.qeye(2)] * N 
            op_list[i] = qt.sigmax().to(data_type)
            sx_list.append(qt.tensor(op_list))
            op_list[i] = qt.sigmay().to(data_type)
            sy_list.append(qt.tensor(op_list))
            op_list[i] = qt.sigmaz().to(data_type)
            sz_list.append(qt.tensor(op_list))

        # Hamiltonian - Energy splitting terms
        H_0 = 0.
        for i in range(N):
            H_0 += g0 * sz_list[i]

        # Interaction terms
        H_1 = qt.qzero_like(H_0)
        for n in range(N - 1):
            H_1 += -J0 * sx_list[n] * sx_list[n + 1]

        # Driving terms
        if A > 0:
            H_d = 0.
            for i in range(N):
                H_d += A * sx_list[i]
            args = {'w': omega}
            H = [H_0, H_1, [H_d, lambda t, w: np.sin(w * t)]]
        else:
            args = {}
            H = [H_0, H_1]

        # Defining initial conditions
        state_list = [qt.basis(2, 1)] * (N-1)
        state_list.append(qt.basis(2, 0))
        psi0 = qt.tensor(state_list)

        # Defining expectation operator
        e_ops = sz_list
        return H, psi0, e_ops, args

options = {"progress_bar": False,
           "store_floquet_states": True}

H, psi0, e_ops, args = setup_Ising_drive(N, g0, J0, A, omega)


# ======================================================
# Initialization of arrays
# ======================================================
computational_time_floquet = np.ones(tlist.shape) * np.nan
computational_time_sesolve = np.ones(tlist.shape) * np.nan

expect_floquet = np.zeros((N, len(tlist)))
expect_sesolve = np.zeros((N, len(tlist)))


# ======================================================
# Starting simulation
# ======================================================
for n, t in enumerate(tlist):
    # --------------------------------
    # Floquet basis
    # --------------------------------
    tic_f = time.perf_counter()
    if t < T:
        # find the floquet modes for the time-dependent hamiltonian
        floquetbasis = qt.FloquetBasis(H, T, args)
    else:
        floquetbasis = qt.FloquetBasis(H, T, args, precompute=tlist_0)

    # Decomposing inital state into Floquet modes
    f_coeff = floquetbasis.to_floquet_basis(psi0)
    # Obtain evolved state in the original basis
    psi_t = floquetbasis.from_floquet_basis(f_coeff, t)
    p_ex = qt.expect(e_ops, psi_t)
    toc_f = time.perf_counter()

    # Saving data
    computational_time_floquet[n] = toc_f - tic_f

    # --------------------------------
    # sesolve
    # --------------------------------
    tic_f = time.perf_counter()
    output = qt.sesolve(H, psi0, tlist[:n + 1], e_ops=e_ops, args=args)
    p_ex_r = output.expect
    toc_f = time.perf_counter()
    # Saving data
    computational_time_sesolve[n] = toc_f - tic_f

    for i in range(N):
        expect_floquet[i, n] = p_ex[i]
        expect_sesolve[i, n] = p_ex_r[i][-1]


# ======================================================
# Plotting results
# ======================================================
sty = ["-", "--"]
fig, axs = plt.subplots(1, 2, figsize=(13.6, 4.5))
ax = axs[0]
ax.plot(tlist / T, computational_time_floquet, sty[0])
ax.plot(tlist / T, computational_time_sesolve, sty[1])

axs[0].set_yscale("log")
axs[0].set_yticks(np.logspace(-3, -1, 3))
lg = []
for i in range(N):
    axs[1].plot(tlist / T, np.real(expect_floquet[i, :]), sty[0], lw='3.5')
    lg.append(f"n={i+1}")
for i in range(N):
    axs[1].plot(tlist / T, np.real(expect_sesolve[i, :]), sty[1], lw='2.5', color="GREEN")

axs[0].set_xlabel(r'$t \, / \, T$')
axs[1].set_xlabel(r'$t \, / \, T$')
ax.set_ylabel(r'$Computational \; Time,\; [s]$')
axs[1].set_ylabel(r'$\langle \sigma_z^{{(n)}} \rangle$')
ax.legend((r"Floquet", r"sesolve"), frameon=False)
axs[1].legend(lg, frameon=False, ncol=2)
xticks = np.rint(np.linspace(0, N_T, N_T + 1, endpoint=True))
axs[0].set_xticks(xticks)
axs[0].set_xlim([0, N_T])
axs[1].set_xticks(xticks)
axs[1].set_xlim([0, N_T])
txt = f'$N={N}$, $g_0={g0}$, $J_0={J0}$, $A={A}$'
axs[0].text(.0, 1.05, txt, transform=axs[0].transAxes)
axs[0].text(-.15, 1.05, r'(a)', transform=axs[0].transAxes)
axs[1].text(-.15, 1.05, r'(b)', transform=axs[1].transAxes)

fig.show()
fig.savefig('./floquet_speed_test_ising.pdf')


==> qip_renderer.tex <==
from qutip_qip.circuit import QubitCircuit

qc = QubitCircuit(2, num_cbits=1) #Circuit consists of two qubits + one classical register
qc.add_gate("H", 0) #Add a Hadamard on qubit '0'
qc.add_gate("H", 1) #Add a Hadamard on qubit '1'
qc.add_gate("CNOT", 1, 0) #Add a CNOT between 0 and 1
qc.add_measurement("M", targets=[0], classical_store=0) #Add a measurement, store result in classical register

# Visualize the circuit
qc.draw("latex")
qc.draw("text")
qc.draw("matplotlib")

==> qobj.tex <==
import qutip as qt
sz = qt.Qobj([[1, 0], [0, -1]]) 
print(sz)
?\pythonoutput?Quantum object: dims=[[2], [2]], shape=(2, 2), type='oper', dtype=Dense, isherm=True
?\pythonoutput?Qobj data =
?\pythonoutput?[[ 1.  0.]
?\pythonoutput? [ 0. -1.]]

sz = qt.Qobj([[1, 0], [0, -1]]) 
sz2 = sz & sz
print(sz2)
?\pythonoutput?Quantum object: dims=[[2, 2], [2, 2]], shape=(4, 4), type='oper',
?\pythonoutput?                dtype=Dense, isherm=True
?\pythonoutput?Qobj data =
?\pythonoutput?[[ 1.  0.  0.  0.]
?\pythonoutput? [ 0. -1.  0. -0.]
?\pythonoutput? [ 0.  0. -1. -0.]
?\pythonoutput? [ 0. -0. -0.  1.]]

print(sz.data)
?\pythonoutput?Dense(shape=(2, 2), fortran=False)
print(sz.to('CSR').data)
?\pythonoutput?CSR(shape=(2, 2), nnz=2)

==> qoc.tex <==
import numpy as np
import qutip as qt

import qutip_qoc as qoc

# objective
initial = qt.qeye(2) # identity
target  = qt.gates.hadamard_transform()

# energy splitting, tunneling, amplitude damping
omega, delta, gamma = 0.1, 1.0, 0.1
sx, sy, sz = qt.sigmax(), qt.sigmay(), qt.sigmaz()

Hc = [sx, sy, sz] # control operator
Hc = [qt.liouvillian(H) for H in Hc]

Hd = 1 / 2 * (omega * sz + delta * sx) # drift term
Hd = qt.liouvillian(H=Hd, c_ops=[np.sqrt(gamma) * qt.sigmam()])

# combined operator list
H = [Hd, Hc[0], Hc[1], Hc[2]]

# pulse time interval
times = np.linspace(0, np.pi/2, 100)

# run the optimization
res_grape = qoc.optimize_pulses(
    objectives=qoc.Objective(initial, H, target),
    control_parameters={
        "ctrl_x": {
            "guess" : np.sin(times),
            "bounds": [-1, 1]
        },
        "ctrl_y": {
            "guess" : np.cos(times),
            "bounds": [-1, 1]
        },
        "ctrl_z": {
            "guess" : np.tanh(times),
            "bounds": [-1, 1]
        }
    },
    tlist=times,
    algorithm_kwargs={
        "alg": "GRAPE",
        "fid_err_targ": 0.01
    }
)

# ------------------------------------------- CRAB EXAMPLE -------------------------------------------

# c0 * sin(c2*t) + c1 * cos(c2*t) + ...
n_params = 3 # adjust in steps of 3

# run the optimization
res_crab = qoc.optimize_pulses(
    objectives=qoc.Objective(initial, H, target),
    control_parameters={
        "ctrl_x": {
            "guess" : [1 for _ in range(n_params)],
            "bounds": [(-1, 1)] * n_params
        },
        "ctrl_y": {
            "guess" : [1 for _ in range(n_params)],
            "bounds": [(-1, 1)] * n_params
        },
        "ctrl_z": {
            "guess" : [1 for _ in range(n_params)],
            "bounds": [(-1, 1)] * n_params
        }
    },
    tlist=times,
    algorithm_kwargs={
        "alg": "CRAB",
        "fid_err_targ": 0.01,
        "fix_frequency": False
    }
)

# ------------------------------------------- GOAT EXAMPLE -------------------------------------------

def sin(t, c):
    return c[0] * np.sin(c[1] * t)

def grad_sin(t, c, idx):
    if idx == 0: # w.r.t. c0
        return np.sin(c[1] * t)
    if idx == 1: # w.r.t. c1
        return c[0] * np.cos(c[1] * t) * t
    if idx == 2: # w.r.t. time
        return c[0] * np.cos(c[1] * t) * c[1]

# similar to qutip.QobjEvo
H = [Hd] + [[hc, sin, {"grad": grad_sin}] for hc in Hc]

ctrl_parameters = {
    id: {
        "guess":  [1, 0], # c0 and c1
        "bounds": [(-1, 1), (0, 2*np.pi)]
    } for id in ['x', 'y', 'z']
}

# magic kwrd to treat time as optimization variable
ctrl_parameters["__time__"] = {
    "guess": times[len(times) // 2],
    "bounds": [times[0], times[-1]],
}

# run the optimization
res_goat = qoc.optimize_pulses(
    objectives=qoc.Objective(initial, H, target),
    control_parameters=ctrl_parameters,
    tlist=times,
    algorithm_kwargs={
        "alg": "GOAT",
        "fid_err_targ": 0.01,
    }
)

# ------------------------------------------- JOPT EXAMPLE -------------------------------------------

import jax

@jax.jit
def sin_y (t, d, **kwargs):
    return d[0] * jax.numpy.sin(d[1] * t)

@jax.jit
def sin_z (t, e, **kwargs):
    return e[0] * jax.numpy.sin(e[1] * t)

import jax
    
@jax.jit
def sin_x (t, c, **kwargs):
    return c[0] * jax.numpy.sin(c[1] * t)

# same for sin_y and sin_z ...

H = [Hd] + [[Hc[0], sin_x], [Hc[1], sin_y], [Hc[2], sin_z]]

res_jopt = qoc.optimize_pulses(
    objectives=qoc.Objective(initial, H, target),
    control_parameters=ctrl_parameters, 
    tlist=times,
    algorithm_kwargs={
        "alg": "JOPT",
        "fid_err_targ": 0.01,
    }
)

# ------------------------------------------- PLOTS -------------------------------------------

import matplotlib.pyplot as plt
from mpl_setup import *

fig, ax = plt.subplots(1, 3, figsize=(13.6, 4.54))

goat_range = times < res_goat.optimized_params[-1]
jopt_range = times < res_jopt.optimized_params[-1]

for i in range(3):
    ax[i].plot(times, res_grape.optimized_controls[i], ':', label='GRAPE')
    ax[i].plot(times, res_crab.optimized_controls[i], '-.', label='CRAB')
    ax[i].plot(times[goat_range], np.array(res_goat.optimized_controls[i])[goat_range], '-', label='GOAT')
    ax[i].plot(times[jopt_range], np.array(res_jopt.optimized_controls[i])[jopt_range], '--', label='JOPT')

    ax[i].set_xlabel(r"Time $t$")

ax[0].legend(loc=0)
ax[0].set_ylabel(r"Pulse amplitude $c_x(t)$", labelpad=-5)
ax[1].set_ylabel(r"Pulse amplitude $c_y(t)$", labelpad=-5)
ax[2].set_ylabel(r"Pulse amplitude $c_z(t)$", labelpad=-5)
ax[2].set_ylim(-0.2, 1.1) # ensure equal spacing between subplots

plt.savefig("qoc_pulse_plot.pdf")
plt.show()



# ------------------------------------------- FIDELITIES -------------------------------------------

print('GRAPE: ', res_grape.fid_err)
print(res_grape.total_seconds, ' seconds')
print()
print('CRAB : ', res_crab.fid_err)
print(res_crab.total_seconds, ' seconds')
print()
print('GOAT : ', res_goat.fid_err)
print(res_goat.total_seconds, ' seconds')
print()
print('JOPT : ', res_jopt.fid_err)
print(res_jopt.total_seconds, ' seconds')

==> qutipqip2.tex <==
#%%
from math import sqrt
import matplotlib.pyplot as plt
import numpy as np

from qutip import basis, tensor
import qutip as qt
qt.settings.core["default_dtype"] = "csr"
from qutip_qip.circuit import QubitCircuit
from qutip_qip.device import SCQubits


# Parameters
epsilon1 = 0.7
epsilon2 = 1.
g = 0.3
tf = 20.  # total time
dt = 2.  # Trotter step size
num_steps = int(tf/dt)

# Hamiltonian we are modelling
sx1 = qt.sigmax() & qt.qeye(2)
sx2 = qt.qeye(2) & qt.sigmax()

sy1 = qt.sigmay() & qt.qeye(2)
sy2 = qt.qeye(2) & qt.sigmay()

sz1 = qt.sigmaz() & qt.qeye(2)
sz2 = qt.qeye(2) & qt.sigmaz()

H = 0.5 * epsilon1 * sz1 + 0.5 * epsilon2 * sz2 + g * sx1 * sx2

init_state = basis(2, 0) & basis(2, 1)


# Exact Schrodinger equation

states_sesolve = qt.sesolve(H, init_state, tlist=np.linspace(0, tf, 100)).states


# Trotterization

trotter_simulation = QubitCircuit(2) #Create circuit consisting of 2 qubits

trotter_simulation.add_gate("RZ", targets=[0], arg_value=(epsilon1 * dt))
trotter_simulation.add_gate("RZ", targets=[1], arg_value=(epsilon2 * dt))

trotter_simulation.add_gate("H", targets=[0]) #Hadamard on qubit 0
trotter_simulation.add_gate("RZX", targets=[0, 1], arg_value=g * dt * 2) #RZX gate
trotter_simulation.add_gate("H", targets=[0]) #Hadamard on qubit 0

trotter_simulation.compute_unitary()
plot1 = trotter_simulation.draw(renderer="matplotlib")
# Evaluate multiple iteration of a circuit
result_circ = init_state
state_trotter_circ = [init_state]

for dd in range(num_steps):
    result_circ = trotter_simulation.run(state=result_circ) #Use previous result as start of next step
    state_trotter_circ.append(result_circ)

# Run pulse-level noisy hardware simulation

processor = SCQubits(num_qubits=2, t1=2e5, t2=2e5) #Superconducting cicuits processor
processor.load_circuit(trotter_simulation) #Load circuit into processor
# Since SCQubit are modelled as qutrit, we need three-level systems here for initial condition:
init_state = tensor(basis(3, 0), basis(3, 1))

state_proc = init_state
state_list_proc = [init_state]
for dd in range(num_steps):
    result = processor.run_state(state_proc)
    state_proc = result.final_state
    state_list_proc.append(result.final_state)


# Plotting

fig, ax = processor.plot_pulses(figsize=(8, 5))
plt.savefig("circuit1.pdf")
fig.show()

plt.figure(figsize=(10, 4.54))
sigmaz_qutrit = qt.basis(3, 0)*qt.basis(3, 0).dag() - qt.basis(3, 1)*qt.basis(3, 1).dag()
plt.plot(np.linspace(0, tf, 100), qt.expect(qt.sigmaz() & qt.qeye(2),states_sesolve), '-',label='Ideal')
plt.plot(np.linspace(0, tf, num_steps + 1), qt.expect(qt.sigmaz() & qt.qeye(2), state_trotter_circ), '--d', label=r'Trotter circuit')
plt.plot(np.linspace(0, tf, num_steps + 1), qt.expect(sigmaz_qutrit & qt.qeye(3), state_list_proc), '-.o',label='noisy hardware')

plt.xlabel('Time', fontsize=18)
plt.ylabel(r'$\langle \sigma_z^{(1)} \rangle$', fontsize=18)

plt.legend(loc=0, fontsize=18, bbox_to_anchor=(1.1, 1.05))
plt.savefig("qip1.pdf")
plt.show()

#%%
# Lindblad simulation
epsilon1 = 0.7
epsilon2 = 1.
g = 0.3
gam = 0.03 # dissipation rate
tf = 20.  # total time
dt = 2.  # Trotter step size
num_steps = int(tf/dt)

# Normal Master equation simulation
init_state_system = qt.tensor(qt.basis(2, 0), qt.basis(2, 1))
tlist = np.linspace(0, tf, 100)
sz1 = qt.tensor(qt.sigmaz(), qt.qeye(2))
sz2 = qt.tensor(qt.qeye(2), qt.sigmaz())

sx1 = qt.tensor(qt.sigmax(), qt.qeye(2))
sx2 = qt.tensor(qt.qeye(2), qt.sigmax())

H = 0.5 * epsilon1 * sz1 + 0.5 * epsilon2 * sz2 + g * sx1 * sx2

# Collapse operators
sm1 = qt.tensor(qt.destroy(2).dag(), qt.qeye(2))
sm2 = qt.tensor(qt.qeye(2), qt.destroy(2).dag())
c_ops = [np.sqrt(gam) * sm1, np.sqrt(gam) * sm2]

result_me = qt.mesolve(
    H, init_state_system, tlist, c_ops,
    e_ops = [tensor([qt.sigmaz(), qt.qeye(2)]), sz2]
    )

# Trotterized circuit simulation
trotter_simulation_noisey = QubitCircuit(4)

# Coherent dynamics
trotter_simulation_noisey.add_gate("RZ",targets=[1], arg_value=epsilon1*dt)
trotter_simulation_noisey.add_gate("RZ",targets=[2], arg_value=epsilon2*dt)

trotter_simulation_noisey.add_gate("H", targets=[1])
trotter_simulation_noisey.add_gate("RZX", targets=[1, 2], arg_value=g*dt*2)
trotter_simulation_noisey.add_gate("H", targets=[1])

# Decoherence
# exp(-i XX t)
trotter_simulation_noisey.add_gate("H", targets=[0])
trotter_simulation_noisey.add_gate("RZX", targets=[0, 1], arg_value=sqrt(gam)*sqrt(dt))
trotter_simulation_noisey.add_gate("H", targets=[0])

# exp(-i YY t)
trotter_simulation_noisey.add_gate("RZ", 1, arg_value=np.pi/2)
trotter_simulation_noisey.add_gate("RX", 0, arg_value=-np.pi/2)
trotter_simulation_noisey.add_gate("RZX", [0, 1], arg_value=sqrt(gam)*sqrt(dt))
trotter_simulation_noisey.add_gate("RZ", 1, arg_value=-np.pi/2)
trotter_simulation_noisey.add_gate("RX", 0, arg_value=np.pi/2)

# exp(-i XX t)
trotter_simulation_noisey.add_gate("H", targets=[2])
trotter_simulation_noisey.add_gate("RZX", targets=[2, 3], arg_value=sqrt(gam)*sqrt(dt))
trotter_simulation_noisey.add_gate("H", targets=[2])

# exp(-i YY t)
trotter_simulation_noisey.add_gate("RZ", 3, arg_value=np.pi/2)
trotter_simulation_noisey.add_gate("RX", 2, arg_value=-np.pi/2)
trotter_simulation_noisey.add_gate("RZX", [2, 3], arg_value=sqrt(gam)*sqrt(dt))
trotter_simulation_noisey.add_gate("RZ", 3, arg_value=-np.pi/2)
trotter_simulation_noisey.add_gate("RX", 2, arg_value=np.pi/2)
trotter_simulation_noisey.draw(renderer="matplotlib")

state_system = qt.ket2dm(init_state_system)
state_trotter_circ = [init_state_system]
for dd in range(num_steps):
    state_full = tensor(
        basis(2, 1)*basis(2, 1).dag(),
        state_system,
        basis(2, 1)*basis(2, 1).dag()
        )
    state_full = trotter_simulation_noisey.run(state=state_full)
    state_system = state_full.ptrace([1, 2])
    state_trotter_circ.append(state_system)
    

# plot results 
times_circ = np.arange(0, tf + dt, dt)
plt.figure()
plt.plot(tlist, result_me.expect[0], '-', label=r'Ideal')
plt.plot(times_circ, qt.expect(qt.tensor(qt.sigmaz(), qt.qeye(2)), state_trotter_circ), "--d", lw=2, label=r'trotter')
plt.xlabel('Time', fontsize=18)
plt.ylabel('Expectation values', fontsize=18)
plt.legend()
plt.show()


#%% Pulse-level noisy hardware simulation, takes ~20 min
processor = SCQubits(num_qubits=4, t1=3.e4, t2=3.e4)
processor.load_circuit(trotter_simulation_noisey)
init_state_system = tensor(basis(3, 0), basis(3, 1))
fig, ax = processor.plot_pulses(figsize=(8, 5))
plt.savefig("circuit2.pdf")
fig.show()

state_system = qt.ket2dm(init_state_system)
state_list_proc = [state_system]
for dd in range(num_steps):
    state_full = tensor(
            basis(3, 1) * basis(3, 1).dag(),
            state_system,
            basis(3, 1) * basis(3, 1).dag(),
            )
    result_noisey = processor.run_state(
        state_full,
        solver="mesolve",
        options={
            "store_states": False,
            "store_final_state": True,
        }
        )
    state_full = result_noisey.final_state
    state_system = state_full.ptrace([1,2])
    state_list_proc.append(state_system)
    print(f"Step {dd+1}/{num_steps} finished.")


times_circ = np.arange(0, tf + dt, dt)
#%%
plt.figure()
plt.plot(tlist, result_me.expect[0],'-', label=r'Ideal')
plt.plot(times_circ, qt.expect(qt.sigmaz() & qt.qeye(2), state_trotter_circ),
         "--d", label=r'Trotter circuit')
plt.plot(times_circ,
         qt.expect(sigmaz_qutrit & qt.qeye(3), state_list_proc),
         "-.o",
         label=r'noisy hardware')

plt.xlabel('Time$', fontsize=18)
plt.ylabel(r'$\langle \sigma_z^{(1)} \rangle$', fontsize=18)
plt.legend()

plt.savefig("qip2.pdf")
plt.show()



==> smesolve.tex <==
import matplotlib.pyplot as plt
from mpl_setup import * 

import qutip as qt
import numpy as np


# parameters
N = 20                 # Hilbert space dimension
delta = 5 * 2 * np.pi  # cavity detuning
kappa = 1              # cavity decay rate
A = 4                  # intensity of initial state
num_traj = 500

# operators
a = qt.destroy(N)
x = a + a.dag()
H = delta * a.dag() * a

rho_0 = qt.coherent(N, np.sqrt(A))
times = np.arange(0, 1, 0.0025)

stoc_solution = qt.smesolve(
    H, rho_0, times, c_ops=[], sc_ops=[np.sqrt(kappa) * a], e_ops=[x],
    ntraj=num_traj, options={"dt": 0.00125, "store_measurement": True}
)

me_solution = qt.mesolve(H, rho_0, times, c_ops=[np.sqrt(kappa) * a], e_ops=[x])

plt.figure()
plt.plot(times[1:], np.array(stoc_solution.measurement).mean(axis=0)[0, :].real,
         lw=2, label=r'$J_x$')
plt.plot(times, stoc_solution.expect[0],
         label=r'$\langle x \rangle$')
plt.plot(times, me_solution.expect[0], '--', color=GRAY,
         label=r'$\langle x \rangle$ mesolve')

plt.xlabel('Time', fontsize=18)
plt.legend()
plt.savefig("smesolve.pdf")
plt.show()

==> solver.tex <==
import qutip as qt
import numpy as np

epsilon1 = 1.0 #qubit 1 energy
epsilon2 = 1.0 #qubit 2 energy
g = 0.1 #coupling strength

sx1 = qt.sigmax() & qt.qeye(2)
sx2 = qt.qeye(2) & qt.sigmax()
sz1 = qt.sigmaz() & qt.qeye(2)
sz2 = qt.qeye(2) & qt.sigmaz()
#Hamiltonian 
H = (epsilon1 / 2) * sz1 + (epsilon2 / 2) * sz2 + g * sx1 * sx2

print(H)
?\pythonoutput?Quantum object: dims=[[2, 2], [2, 2]], shape=(4, 4), type='oper',
?\pythonoutput?                dtype=CSR, isherm=True
?\pythonoutput?Qobj data =
?\pythonoutput?[[ 1.   0.   0.   0.1]
?\pythonoutput? [ 0.   0.   0.1  0. ]
?\pythonoutput? [ 0.   0.1  0.   0. ]
?\pythonoutput? [ 0.1  0.   0.  -1. ]]

psi0 = qt.basis(2, 0) & qt.basis(2, 1) #initial state
tlist = np.linspace(0, 40, 100) #time steps
result = qt.sesolve(H, psi0, tlist) #solver result

solver = qt.SESolver(H) #create solve object
result2 = solver.run(psi0, tlist) #get result from solver object

t = 0
dt = 40 / 100
solver.start(psi0, t)
while t < 40:
    t = t + dt
    psi = solver.step(t)
    dt = ... # process the result psi and calculate the next time step

options = {"store_states": True, "atol": 1e-12, "nsteps": 1000, "max_step": 0.1}
solver.options = options
result3 = solver.run(psi0, tlist)  # Or: qt.sesolve(H, psi0, tlist, options=options)
print(result3)
?\pythonoutput?<Result
?\pythonoutput?  Solver: sesolve
?\pythonoutput?  Solver stats:
?\pythonoutput?    method: 'scipy zvode adams'
?\pythonoutput?    init time: 3.5762786865234375e-05
?\pythonoutput?    preparation time: 0.0001609325408935547
?\pythonoutput?    run time: 0.007315397262573242
?\pythonoutput?    solver: 'Schrodinger Evolution'
?\pythonoutput?  Time interval: [0.0, 40.0] (100 steps)
?\pythonoutput?  Number of e_ops: 0
?\pythonoutput?  States saved.
?\pythonoutput?>

==> tutorial_snippets.tex <==
#this is not a compilable file,just a collection of snippets from the tutorials to import to the text

def cos_t(t):
    return np.cos(t)
function_form = (n + (a + ad) * qutip.coefficient(cos_t))





tlist = np.linspace(0, 10, 101)
values = np.cos(tlist)

array_form = (n + (a + ad) * qutip.coefficient(values, tlist=tlist))



args = {"state": qutip.MESolver.StateFeedback(default=qutip.fock_dm(4, 2))}
def print_args(t, state):
    print(f"'state':\n{state}")
    return t + state.norm()
td_args = qutip.QobjEvo([Id, print_args], args=args)

